Multimodal C4: An Open, Billion-scale Corpus of Images Interleaved with Text

In-context vision and language models like Flamingo support arbitrarily interleaved sequences of images and text as input. This format not only enables few-shot learning via interleaving independent supervised (image, text) examples, but also, more complex prompts involving interaction between images, e.g., "What do image A and image B have in common?" To support this interface, pretraining occurs over web corpora that similarly contain interleaved images+text. To date, however, large-scale data of this form have not been publicly available. We release Multimodal C4, an augmentation of the popular text-only C4 corpus with images interleaved. We use a linear assignment algorithm to place images into longer bodies of text using CLIP features, a process that we show outperforms alternatives. Multimodal C4 spans everyday topics like cooking, travel, technology, etc. A manual inspection of a random sample of documents shows that a vast majority (88%) of images are topically relevant, and that linear assignment frequently selects individual sentences specifically well-aligned with each image (80%). After filtering NSFW images, ads, etc., the resulting corpus consists of 101.2M documents with 571M images interleaved in 43B English tokens.

==> sections/A0-checklist.tex <==
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See \url{https://github.com/allenai/mmc4/blob/main/DATASET_CARD.md#other-known-limitations}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See \url{https://github.com/allenai/mmc4/blob/main/DATASET_CARD.md#social-impact-of-dataset}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See \url{https://github.com/allenai/mmc4/}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{The \cfour dataset~\cite{raffel2020exploring} has Apache License, and the term of use for Common Crawl can be found at \url{https://commoncrawl.org/terms-of-use/full/}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See \url{https://github.com/allenai/mmc4/}.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{See \S~\ref{sec:sec_with_data_collection}.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See \S~\ref{sec:sec_with_data_release_considerations}.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

% \clearpage

==> tables/flamingo_results_as_table.tex <==
\begin{table}[htbp]
  \centering
  \begin{tabular}{l|ccc}
    \toprule
    Pre-training data & 0-shot* & 4-shot & 8-shot \\
    \midrule
    % LAION-2B (5M samples) & 18.30 & 10.64 & 9.06 \\
    LAION-2B (5M ex) & 18.3 & 10.6 & 9.1 \\
    % $\rotatebox[origin=c]{180}{$\Lsh$}$ + \mmcfourcore (2.5M samples) & 17.36 & 46.49 & 48.56 \\
    $\rotatebox[origin=c]{180}{$\Lsh$}$ + \mmcfourcore (2.5M ex) & 17.4 & 46.5 & 48.6 \\
    % LAION-2B (10M samples) & 24.15 & 27.22 & 14.44 \\
    LAION-2B (10M ex) & 24.2 & 27.2 & 14.4 \\
    % $\rotatebox[origin=c]{180}{$\Lsh$}$ + \mmcfourcore (5M samples) & 18.18 & 58.54 & 59.07 \\
    $\rotatebox[origin=c]{180}{$\Lsh$}$ + \mmcfourcore (5M ex) & 18.2 & 58.5 & 59.1 \\
    % LAION-2B (15M samples) & 25.17 & 40.25 & 23.90 \\
    LAION-2B (15M ex) & 25.2 & 40.3 & 23.9 \\
     % $\rotatebox[origin=c]{180}{$\Lsh$}$ + \mmcfourcore (7.5M samples) & 17.93 & 60.25 & 61.24 \\
     $\rotatebox[origin=c]{180}{$\Lsh$}$ + \mmcfourcore (7.5M ex) & 17.9 & 60.3 & 61.2 \\
    \bottomrule
  \end{tabular}
  \vspace{5px}
  \caption{Pretraining corpus ablation: MSCOCO \cite{lin2014microsoft} caption generation performance (Val CIDEr \cite{vedantam2015cider}) of OpenFlamingo-3B (OPT-1.3B/CLIP+ViT-L/14) when pretrained on different corpora. Models trained on \mmcfourcore can better handle interleaved images with text during inference. *0-shot performance is without pre-pending two example captions, c.f. \cite{alayrac2022flamingo}.}
\label{tab:training-exp}
\end{table}

==> tables/image_relevance.tex <==
\begin{table}[t]\centering
% \begin{adjustbox}{width=0.6\textwidth,center}
\begin{tabular}{lrr}\toprule
&Count &Percentage \\
\midrule
Total &799 &100.00\% \\
\midrule
Topically related to the document &715 &89.49\% \\
Aligned to the assigned sentence &620 &77.60\% \\
\midrule
w/ faces & 178 & 22.28\% \\
w/ watermarks & 26 & 3.25\% \\
Logo-related & 33 & 4.13\% \\
Ads-related & 17 & 2.13\% \\
Duplicated & 11 & 1.38\% \\
\bottomrule
\end{tabular}
\vspace{5px}
\caption{Results of manual verification of 200 randomly sampled \mmcfour documents. A majority of images are topically relevant/aligned. The rate of images with potentially undesirable properties (watermarks, ads, duplicates, etc.) is low.
% We manually examined 799 images from 200 randomly sampled \mmcfour documents and report the percentage of images that are topically related to the document and are aligned to the assigned sentence.
% We also report the percentage of images that contain human faces or watermarks, images related to logos or ads, and the duplicated images within the document.
}
\label{tab:image_relevance}
% \end{adjustbox}
\end{table}

==> tables/image_relevance_v2.tex <==
\begin{table}[t]\centering
% \begin{adjustbox}{width=0.6\textwidth,center}
\begin{tabular}{lr}\toprule
%  \multicolumn{2}{r}{\% of 799 images} \\
% \midrule
% Topically-related & 89.5\% \\
% Sentence-aligned & 77.6\% \\
% \midrule
% Has face? & 22.3\% \\
% Has watermark? & 3.3\% \\
% Logo-related & 4.1\% \\
% Ads-related &  2.1\% \\
% Duplicated & 1.4\% \\

 \multicolumn{2}{r}{\% of 834 images} \\
\midrule
Topically-related & ?\% \\
Sentence-aligned & ?\% \\
\midrule
Has face? & 28.4\% \\
Has watermark? & 1.6\% \\
Logo-related & 3.7\% \\
Ads-related &  2.5\% \\
Duplicated & 0.6\% \\

\bottomrule
\end{tabular}
\vspace{5px}
\caption{Results of manual verification of 200 randomly sampled \mmcfour documents containing 799 images. A majority of images are topically relevant and well sentence-aligned. The rate of watermarks, ads, duplicates, etc. is low.
% We manually examined 799 images from 200 randomly sampled \mmcfour documents and report the percentage of images that are topically related to the document and are aligned to the assigned sentence.
% We also report the percentage of images that contain human faces or watermarks, images related to logos or ads, and the duplicated images within the document.
}
\label{tab:image_relevance}
% \end{adjustbox}
\end{table}
